Will this Question be Answered? Question Filtering via Answer Model Distillation for Efficient Question Answering

In this paper we propose a novel approach towards improving the efficiency of Question Answering (QA) systems by filtering out questions that will not be answered by them. This is based on an interesting new finding: the answer confidence scores of state-of-the-art QA systems can be approximated well by models solely using the input question text. This enables preemptive filtering of questions that are not answered by the system due to their answer confidence scores being lower than the system threshold. Specifically, we learn Transformer-based question models by distilling Transformer-based answering models. Our experiments on three popular QA datasets and one industrial QA benchmark demonstrate the ability of our question models to approximate the Precision/Recall curves of the target QA system well. These question models, when used as filters, can effectively trade off lower computation cost of QA systems for lower Recall, e.g., reducing computation by ~60%, while only losing ~3-4% of Recall.

==> EMNLP'21 Question Filtering/Tables/baselines.tex <==
\begin{table}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{ccccccc}
\toprule
\multirow{2}{*}{\textbf{{\TM} of {\M} $\downarrow$}}  & & \multicolumn{2}{c}{{\FW}} & &\multicolumn{2}{c}{{\FC}} \\ \cmidrule{3-4} \cmidrule{6-7}
& & Base & Large & & Base & Large \\
\midrule
0.3 & & 0.3 / \textcolor{red}{\contour{red}{-}}0.1 & 0.1 / \textcolor{red}{\contour{red}{-}}0.2 & & 	0.2 / \textcolor{red}{\contour{red}{-}}0.1 & 0.3 / \textcolor{red}{\contour{red}{-}}0.2 \\


0.5 & & 0.9 / \textcolor{red}{\contour{red}{-}}0.4 & 0.1 / \textcolor{red}{\contour{red}{-}}0.1 && 1.0 / \textcolor{red}{\contour{red}{-}}0.2 & 0.5 / \textcolor{red}{\contour{red}{-}}0.3 \\


0.6 && 0.9 / \textcolor{red}{\contour{red}{-}}0.4 & 0.1 / \textcolor{red}{\contour{red}{-}}0.2 && 22.3 / \textcolor{red}{\contour{red}{-}}5.0 & 2.7 / \textcolor{red}{\contour{red}{-}}0.8 \\


0.7 && 1.0 / \textcolor{red}{\contour{red}{-}}0.2 & 0.2 / \textcolor{red}{\contour{red}{-}}0.1 && 38.5 / \textcolor{red}{\contour{red}{-}}6.2 & 7.2 / \textcolor{red}{\contour{red}{-}}1.3 \\

0.9 && 0 / 0 & 0 / 0 && 84.4 / \textcolor{red}{\contour{red}{-}}4.8 & 62.5 / \textcolor{red}{\contour{red}{-}}8.1 \\ \bottomrule
\end{tabular}
}
\vspace{-8pt}
\caption{$\%$ Filter / $\Delta$ Recall results of baseline question filters {\FW} and {\FC} at optimal {\TFBest} on ASNQ. Metrics are similar to those in Table~\ref{tab:main_table_small}. Base and Large refers to RoBERTa-Base and RoBERTa-Large question filters.} 
\label{tab:baselines}
\end{table}

==> EMNLP'21 Question Filtering/Tables/error_analysis.tex <==
\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{ccc}
\toprule
\textbf{Question} & {\F} & {\M} \\ \midrule
%  Is it possible to have a body temperature less than 98.6?
1. What's your favorite movie series? & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} \\
2. Where is the key to the building? & \textcolor{red}{\xmark} & \textcolor{red}{\xmark} \\
3. Was Jennifer Lopez a cheerleader for the Lakers? & \textcolor{darkgreen}{\cmark} & \textcolor{red}{\xmark} \\
4. What are two things that all horses have? & \textcolor{darkgreen}{\cmark} & \textcolor{red}{\xmark} \\
5. Which mayors of New York City had the name David? & \textcolor{red}{\xmark} & \textcolor{darkgreen}{\cmark} \\
6. Does Ahsoka Tano appear in the Mandalorian? & \textcolor{red}{\xmark} & \textcolor{darkgreen}{\cmark} \\
\bottomrule
\end{tabular}
}
\vspace{-8pt}
\caption{Qualitative examples of questions along with the filtering decision of {\M}$\langle 0.5 \rangle$ and {\FM}$\langle 0.5 \rangle$ (\textcolor{darkgreen}{\cmark} / \textcolor{red}{\xmark} indicates clearing / failing the threshold).} 
\label{tab:error_analysis}
\end{table}

==> EMNLP'21 Question Filtering/Tables/main_table.tex <==
\begin{table*}[t]
%\hspace{-2.5em}
\resizebox{\linewidth}{!}{
\begin{tabular}{cccccccccccccc}

\multicolumn{3}{c}{\multirow{2}{*}{}}                           & \multicolumn{5}{c}{\textbf{{\M} : 12-Layer Transformer Architecture, {\F} : RoBERTa-Base}}                                                                                                             &   & \multicolumn{5}{c}{\textbf{{\M} : 24-Layer Transformer Architecture, {\F} : RoBERTa-Large}}                                                                                                                              \\ \cmidrule{4-8} \cmidrule{10-14} 
\multicolumn{3}{c}{\textbf{Threshold {\TM} for {\M} $\rightarrow$}}    & \multicolumn{1}{c}{0.3} & \multicolumn{1}{c}{0.5} & \multicolumn{1}{c}{0.6} & \multicolumn{1}{c}{0.7} & 0.9  &     & \multicolumn{1}{c}{0.3} & \multicolumn{1}{c}{0.5} & \multicolumn{1}{c}{0.6} & \multicolumn{1}{c}{0.7} & \multicolumn{1}{c}{0.9} \\ \toprule
\multirow{6}{*}{\begin{turn}{90}\textbf{WikiQA}\end{turn}} & \multirow{2}{*}{{\MTM}} & Pr / Re       	& 84.4  /  80.2 &	87.1  /  75.3 & 88.4  /  68.7 & 88.4  /  63.0 &	97.1  /  28.0 & & 92.1  /  86.0	& 92.2 / 83.1	& 92.0 / 80.2	& 92.1 / 77.0 &	95.9 / 57.2          \\ \cline{3-3}
                      &                           & F1          	& 82.2	& 80.8 & 77.3 & 	73.6	& 43.5  &   & 89.9 &	87.4 &	85.7 &	83.9 &	71.7    \\ \cmidrule{2-3}
                                          & \multirow{2}{*}{\small{\FMTM${\langle{\tau_2^*}\rangle}{\rightarrow}${\M}$\langle${\TM}$\rangle$}}         & $\Delta$ Pr / $\Delta$ Re           & \textcolor{red}{\contour{red}{-}}0.3  /  \textcolor{red}{\contour{red}{-}}2.4  & \textcolor{darkgreen}{\contour{darkgreen}{+}}0.3  / \textcolor{red}{\contour{red}{-}} 0.8  & \textcolor{red}{\contour{red}{-}}0.3  / \textcolor{red}{\contour{red}{-}}1.6  & \textcolor{darkgreen}{\contour{darkgreen}{+}}0.7  /  \textcolor{red}{\contour{red}{-}}2.5  & \textcolor{red}{\contour{red}{-}}0.4  / \textcolor{red}{\contour{red}{-}} 3.7 &  &  \textcolor{red}{\contour{red}{-}}0.1  /  \textcolor{red}{\contour{red}{-}}0.8  & \textcolor{darkgreen}{\contour{darkgreen}{+}}0.3  /  \textcolor{red}{\contour{red}{-}}2.0  & \textcolor{darkgreen}{\contour{darkgreen}{+}}0.5  / \textcolor{red}{\contour{red}{-}} 4.1  & \textcolor{red}{\contour{red}{-}}0.5  / \textcolor{red}{\contour{red}{-}} 5.0  & \textcolor{darkgreen}{\contour{darkgreen}{+}}0.2 / \textcolor{red}{\contour{red}{-}}6.1      \\ \cline{3-3}
                      &                           & $\%$ Filter / $\Delta$ F1 & 	4.1 / \textcolor{red}{\contour{red}{-}}0.9 &	2.9 / \textcolor{red}{\contour{red}{-}}0.4 & 3.7 / \textcolor{red}{\contour{red}{-}}1.1	&7.0 / \textcolor{red}{\contour{red}{-}}1.5 &	42.8 / \textcolor{red}{\contour{red}{-}} 4.7 &   &  0.8 / \textcolor{red}{\contour{red}{-}}0.4  & 3.3 / \textcolor{red}{\contour{red}{-}} 1.0  & 6.6 / \textcolor{red}{\contour{red}{-}} 2.2  & 7.8 / \textcolor{red}{\contour{red}{-}} 3.3  & 18.9 / \textcolor{red}{\contour{red}{-}} 4.1 \\ \cmidrule{2-3}
                     & \multirow{2}{*}{\small{\FM${\langle{\tau_2^*}\rangle}{\rightarrow}${\M}$\langle${\TM}$\rangle$}}         & $\Delta$ Pr / $\Delta$ Re   & \textcolor{darkgreen}{\contour{darkgreen}{+}}0.7  / \textcolor{red}{\contour{red}{-}}2.8  & \textcolor{darkgreen}{\contour{darkgreen}{+}}2.3  /  \textcolor{red}{\contour{red}{-}}10.3  & \textcolor{darkgreen}{\contour{darkgreen}{+}}2.8  / \textcolor{red}{\contour{red}{-}} 9.0  & \textcolor{darkgreen}{\contour{darkgreen}{+}}3.3  / \textcolor{red}{\contour{red}{-}}8.3  & \textcolor{red}{\contour{red}{-}}0.9  / \textcolor{red}{\contour{red}{-}}7.4 &   &  \textcolor{red}{\contour{red}{-}}0.1  / \textcolor{red}{\contour{red}{-}}0.8  & 0  / \textcolor{red}{\contour{red}{-}}0.8  & \textcolor{red}{\contour{red}{-}}0.1  / \textcolor{red}{\contour{red}{-}}0.4  & \textcolor{red}{\contour{red}{-}}0.2  / \textcolor{red}{\contour{red}{-}}2.1  & \textcolor{red}{\contour{red}{-}}0.2  / \textcolor{red}{\contour{red}{-}}2.9  \\ \cline{3-3}
                      &                           & $\%$ Filter / $\Delta$ F1 &  4.1 / \textcolor{red}{\contour{red}{-}} 1.1 &	17.3 / \textcolor{red}{\contour{red}{-}} 5.0 & 20.9 / \textcolor{red}{\contour{red}{-}} 5.1 &	21.0 / \textcolor{red}{\contour{red}{-}}5.1 &	44.0 / \textcolor{red}{\contour{red}{-}} 9.6  &    &  1.2 / \textcolor{red}{\contour{red}{-}}1.4  & 1.8 / \textcolor{red}{\contour{red}{-}}0.4  & 2.6 / \textcolor{red}{\contour{red}{-}}0.3  & 3.9 / \textcolor{red}{\contour{red}{-}}1.4  & 8.8 / \textcolor{red}{\contour{red}{-}}2.4                  \\ \midrule
%%%%%%%%%%%New Dataset
\multirow{6}{*}{\begin{turn}{90}\textbf{ASNQ}\end{turn}} & \multirow{2}{*}{{\MTM}} & Pr / Re                & 68.2  /  48.7                & 74.6  /  41.1                &           77.2  /  36.1              & 79.6  /  28.9      & 90.5  /  10.0 &   & 75.7  /  61.1               & 79.6  /  54.4    &         81.9  /  49.3            & 84.5  /  42.7               & 92.9  /  20.7     \\ \cline{3-3}
                      &                           & F1                               & 56.8                     & 53.0                     &                 49.2         & 42.4                     & 18.0   &           & 67.6                     & 64.6                     &         61.5        & 56.7                    & 33.9      \\ \cmidrule{2-3}
                                          & \multirow{2}{*}{\small{\FMTM${\langle{\tau_2^*}\rangle}{\rightarrow}${\M}$\langle${\TM}$\rangle$}}         & $\Delta$ Pr / $\Delta$ Re         & \textcolor{darkgreen}{\contour{darkgreen}{+}}0.9  / \textcolor{red}{\contour{red}{-}}1.8                & \textcolor{darkgreen}{\contour{darkgreen}{+}}1.6  / \textcolor{red}{\contour{red}{-}}2.9               &     \textcolor{darkgreen}{\contour{darkgreen}{+}}1.6  /  \textcolor{red}{\contour{red}{-}}4.7  & \textcolor{darkgreen}{\contour{darkgreen}{+}}2.5 / \textcolor{red}{\contour{red}{-}}8.2                & \textcolor{darkgreen}{\contour{darkgreen}{+}}0.6  /  \textcolor{red}{\contour{red}{-}}3.9  &  & 0  /  0                              & \textcolor{darkgreen}{\contour{darkgreen}{+}}1.3  / \textcolor{red}{\contour{red}{-}} 3.2  &     \textcolor{darkgreen}{\contour{darkgreen}{+}}1.5  / \textcolor{red}{\contour{red}{-}}3.0           & \textcolor{darkgreen}{\contour{darkgreen}{+}}1.8  / \textcolor{red}{\contour{red}{-}}7.4               & \textcolor{darkgreen}{\contour{darkgreen}{+}}2.4 / \textcolor{red}{\contour{red}{-}}7.0                \\ \cline{3-3}
                      &                           & $\%$ Filter / $\Delta$ F1 &  7.8 / \textcolor{red}{\contour{red}{-}}0.9                      & 17.8 / \textcolor{red}{\contour{red}{-}}2.1                     &                 29.8 / \textcolor{red}{\contour{red}{-}}4.3         & 54.2 / \textcolor{red}{\contour{red}{-}}9.3                     & 83.8 / \textcolor{red}{\contour{red}{-}}6.6   &   &  0.2 / 0                      & 10.5 / \textcolor{red}{\contour{red}{-}}1.9                     &   15.6 / \textcolor{red}{\contour{red}{-}}2.0              & 29.8 / \textcolor{red}{\contour{red}{-}}6.6                     & 66.2 / \textcolor{red}{\contour{red}{-}}9.9                     \\ \cmidrule{2-3}
           & \multirow{2}{*}{\small{\FM${\langle{\tau_2^*}\rangle}{\rightarrow}${\M}$\langle${\TM}$\rangle$}}         & $\Delta$ Pr / $\Delta$ Re         &  \textcolor{darkgreen}{\contour{darkgreen}{+}}0.7 /  \textcolor{red}{\contour{red}{-}}1.2  & \textcolor{darkgreen}{\contour{darkgreen}{+}}0.6  /  \textcolor{red}{\contour{red}{-}}2.7  & \textcolor{darkgreen}{\contour{darkgreen}{+}}1.4  /  \textcolor{red}{\contour{red}{-}}5.3  & \textcolor{darkgreen}{\contour{darkgreen}{+}}1.9  / \textcolor{red}{\contour{red}{-}}6.4  & \textcolor{red}{\contour{red}{-}}1.3 / \textcolor{red}{\contour{red}{-}}5.1 &  &  \textcolor{darkgreen}{\contour{darkgreen}{+}}0.2  /  \textcolor{red}{\contour{red}{-}}0.1  & \textcolor{darkgreen}{\contour{darkgreen}{+}}0.8  /  \textcolor{red}{\contour{red}{-}}3.3  & \textcolor{darkgreen}{\contour{darkgreen}{+}}1.0  /  \textcolor{red}{\contour{red}{-}}3.5  & \textcolor{darkgreen}{\contour{darkgreen}{+}}1.4  / \textcolor{red}{\contour{red}{-}}3.9  & \textcolor{darkgreen}{\contour{darkgreen}{+}}2.2  /  \textcolor{red}{\contour{red}{-}}6.3                \\ \cline{3-3}
                      &                           & $\%$ Filter / $\Delta$ F1 &  6.0 / \textcolor{red}{\contour{red}{-}}0.4                      & 14.9 / \textcolor{red}{\contour{red}{-}}2.2                     &       33.5 / \textcolor{red}{\contour{red}{-}}4.9                   & 47.1 / \textcolor{red}{\contour{red}{-}}7.1                     & 86.0 / \textcolor{red}{\contour{red}{-}}8.7  &    &  1.0 / 0                      & 12.1 / \textcolor{red}{\contour{red}{-}}2.1                     &         16.1 / \textcolor{red}{\contour{red}{-}}2.5                 & 21.6 / \textcolor{red}{\contour{red}{-}}3.2                     & 61.6 / \textcolor{red}{\contour{red}{-}}8.9                     \\ \midrule

%%%%%%%%%%%New Dataset
\multirow{6}{*}{\begin{turn}{90}\textbf{SQuAD 1.1}\end{turn}} & \multirow{2}{*}{{\MTM}} & Pr / Re         &     	82.0  /  75.0  & 	88.7 / 63.3 & 	91.0  /  54.6 & 93.4  /  45.9 & 	96.7  /  28.7 &  & 	86.0 / 82.9 & 	90.1 / 75.3 & 	92.3 / 67.5 & 	94.4 / 59.7 & 	97.6 / 42.4         \\ \cline{3-3}
                      &                           & F1             & 78.3 & 	73.9 &	68.3 &	61.6 & 44.3   &   &     	84.4 & 	82.0 & 	78.0 & 	73.1 & 	59.1          \\ \cmidrule{2-3}
            & \multirow{2}{*}{\small{\FMTM${\langle{\tau_2^*}\rangle}{\rightarrow}${\M}$\langle${\TM}$\rangle$}}         & $\Delta$ Pr / $\Delta$ Re         & 0 / 0  & \textcolor{darkgreen}{\contour{darkgreen}{+}}0.3  / \textcolor{red}{\contour{red}{-}} 2.3  & \textcolor{darkgreen}{\contour{darkgreen}{+}}0.4  / \textcolor{red}{\contour{red}{-}}2.4  & \textcolor{darkgreen}{\contour{darkgreen}{+}}0.6  / \textcolor{red}{\contour{red}{-}}4.8  & \textcolor{darkgreen}{\contour{darkgreen}{+}}0.1  /  \textcolor{red}{\contour{red}{-}}7.7  &   &  0 / 0  & \textcolor{darkgreen}{\contour{darkgreen}{+}}0.1  / \textcolor{red}{\contour{red}{-}}0.5  & \textcolor{darkgreen}{\contour{darkgreen}{+}}0.3  / \textcolor{red}{\contour{red}{-}}1.8  & \textcolor{darkgreen}{\contour{darkgreen}{+}}0.5 / \textcolor{red}{\contour{red}{-}}3.8 & 	\textcolor{darkgreen}{\contour{darkgreen}{+}}0.3 / \textcolor{red}{\contour{red}{-}}3.7               \\ \cline{3-3}
                      &                           & $\%$ Filter / $\Delta$ F1  &	0 / 0	 & 9.4 / \textcolor{red}{\contour{red}{-}}1.5 &	12.9 / \textcolor{red}{\contour{red}{-}}1.9 &	27.4 / \textcolor{red}{\contour{red}{-}}4.4 &	61.0 / \textcolor{red}{\contour{red}{-}}9.8 &  &	0 / 0 &	2.0 / \textcolor{red}{\contour{red}{-}}0.2 &	6.4 / \textcolor{red}{\contour{red}{-}}1.1	&14.0 / \textcolor{red}{\contour{red}{-}}2.7 &	47.5 / \textcolor{red}{\contour{red}{-}}3.7 \\ \cmidrule{2-3}
            & \multirow{2}{*}{\small{\FM${\langle{\tau_2^*}\rangle}{\rightarrow}${\M}$\langle${\TM}$\rangle$}}         & $\Delta$ Pr / $\Delta$ Re           & \textcolor{darkgreen}{\contour{darkgreen}{+}}0.2  / \textcolor{red}{\contour{red}{-}}0.4  & \textcolor{darkgreen}{\contour{darkgreen}{+}}0.5  /  \textcolor{red}{\contour{red}{-}}2.3  & \textcolor{darkgreen}{\contour{darkgreen}{+}}0.6  /  \textcolor{red}{\contour{red}{-}}3.2  & \textcolor{darkgreen}{\contour{darkgreen}{+}}0.7  /  \textcolor{red}{\contour{red}{-}}8.2  & \textcolor{darkgreen}{\contour{darkgreen}{+}}0.2  / \textcolor{red}{\contour{red}{-}}8.8 &      & 0  /  0 & \textcolor{darkgreen}{\contour{darkgreen}{+}}0.1  / \textcolor{red}{\contour{red}{-}}0.5  & \textcolor{darkgreen}{\contour{darkgreen}{+}}0.3 / \textcolor{red}{\contour{red}{-}}1.2 & \textcolor{darkgreen}{\contour{darkgreen}{+}}0.7  / \textcolor{red}{\contour{red}{-}}5.5  & \textcolor{darkgreen}{\contour{darkgreen}{+}}0.3  /  \textcolor{red}{\contour{red}{-}}8.1  \\ \cline{3-3}
                      &                           & $\%$ Filter / $\Delta$ F1  &	1.1 / \textcolor{red}{\contour{red}{-}}0.1 &	9.0 / \textcolor{red}{\contour{red}{-}}1.4 & 	14.2 / \textcolor{red}{\contour{red}{-}}2.5 & 	36.5 / \textcolor{red}{\contour{red}{-}}7.8 & 	63.0 / \textcolor{red}{\contour{red}{-}}10.3  & &    	0 / 0 &	2.4 / \textcolor{red}{\contour{red}{-}}0.3 &	5.1 / \textcolor{red}{\contour{red}{-}}0.7 &	18.2 / \textcolor{red}{\contour{red}{-}}4.1 & 41.8 / \textcolor{red}{\contour{red}{-}}8.3                \\ \midrule 
\multirow{5}{*}{\begin{turn}{90}\textbf{AQAD} \end{turn}} & {\MTM} & Pr / Re         &  	{$\uparrow$}9.2 / {$\downarrow$}4.5 & 	{$\uparrow$}17.9 / {$\downarrow$}12.1 & 	{$\uparrow$}23.4 / {$\downarrow$}15.7 & 	{$\uparrow$}28.1 / {$\downarrow$}20.1 & 	{$\uparrow$}43.0 / {$\downarrow$}31.9 &  &  	{$\uparrow$}9.2 / {$\downarrow$}4.5 & 	{$\uparrow$}17.9 / {$\downarrow$}12.1 & 	{$\uparrow$}23.4 / {$\downarrow$}15.7 & 	{$\uparrow$}28.1 / {$\downarrow$}20.1 & 	{$\uparrow$}43.0 / {$\downarrow$}31.9     \\ 
             \cmidrule{2-3}
     & \multirow{2}{*}{\small{\FMTM${\langle{\tau_2^*}\rangle}{\rightarrow}${\M}$\langle${\TM}$\rangle$}}         & $\Delta$ Pr / $\Delta$ Re           & \textcolor{darkgreen}{\contour{darkgreen}{+}}1.3  /  \textcolor{red}{\contour{red}{-}}3.4  & \textcolor{darkgreen}{\contour{darkgreen}{+}}1.9  /  \textcolor{red}{\contour{red}{-}}5.0  & \textcolor{darkgreen}{\contour{darkgreen}{+}}2.0  /  \textcolor{red}{\contour{red}{-}}5.6  & \textcolor{darkgreen}{\contour{darkgreen}{+}}1.2  /  \textcolor{red}{\contour{red}{-}}6.0  & \textcolor{red}{\contour{red}{-}}1.9  /  \textcolor{red}{\contour{red}{-}}3.4 & 
   &  \textcolor{darkgreen}{\contour{darkgreen}{+}}1.8  /  \textcolor{red}{\contour{red}{-}}3.2  &\textcolor{darkgreen}{\contour{darkgreen}{+}}2.5  /  \textcolor{red}{\contour{red}{-}}4.9  & \textcolor{darkgreen}{\contour{darkgreen}{+}}2.3  /  \textcolor{red}{\contour{red}{-}}5.5  & \textcolor{darkgreen}{\contour{darkgreen}{+}}1.8  /  \textcolor{red}{\contour{red}{-}}4.6  & \textcolor{darkgreen}{\contour{darkgreen}{+}}1.9  /  \textcolor{red}{\contour{red}{-}}3.0  \\ \cline{3-3}
                \cline{3-3}
              &                & $\%$ Filter / $\Delta$ F1 &  20.8 / \textcolor{red}{\contour{red}{-}}2.1 & 43.2 / \textcolor{red}{\contour{red}{-}}4.8 &	53.9 / \textcolor{red}{\contour{red}{-}}6.4 &	65.2 / \textcolor{red}{\contour{red}{-}}8.0 &	89.4 / \textcolor{red}{\contour{red}{-}}6.2 &  & 	21.9 / \textcolor{red}{\contour{red}{-}}1.8 &	45.8 / \textcolor{red}{\contour{red}{-}}4.6 &	56.9 / \textcolor{red}{\contour{red}{-}}6.3 &	66.2 / \textcolor{red}{\contour{red}{-}}7.4 &	89.9 / \textcolor{red}{\contour{red}{-}}5.4
 \\ \cmidrule{2-3}
                 & \multirow{2}{*}{\small{\FM${\langle{\tau_2^*}\rangle}{\rightarrow}${\M}$\langle${\TM}$\rangle$}}         & $\Delta$ Pr / $\Delta$ Re          & \textcolor{darkgreen}{\contour{darkgreen}{+}}1.5  /  \textcolor{red}{\contour{red}{-}}2.8  & \textcolor{darkgreen}{\contour{darkgreen}{+}}2.5  /  \textcolor{red}{\contour{red}{-}}6.6  & \textcolor{darkgreen}{\contour{darkgreen}{+}}2.1  /  \textcolor{red}{\contour{red}{-}}7.5  & \textcolor{darkgreen}{\contour{darkgreen}{+}}1.1  /  \textcolor{red}{\contour{red}{-}}8.7  & \textcolor{red}{\contour{red}{-}}4.1  /  \textcolor{red}{\contour{red}{-}}3.8 & 
    & \textcolor{darkgreen}{\contour{darkgreen}{+}}1.3  /  \textcolor{red}{\contour{red}{-}}1.7  & \textcolor{darkgreen}{\contour{darkgreen}{+}}2.7  /  \textcolor{red}{\contour{red}{-}}5.7  & \textcolor{darkgreen}{\contour{darkgreen}{+}}1.9  /  \textcolor{red}{\contour{red}{-}}6.2  & \textcolor{darkgreen}{\contour{darkgreen}{+}}2.3  /  \textcolor{red}{\contour{red}{-}}7.0  & \textcolor{darkgreen}{\contour{darkgreen}{+}}0.2  /  \textcolor{red}{\contour{red}{-}}3.9  \\ \cline{3-3}
     \cline{3-3}
                     &                 & $\%$ Filter / $\Delta$ F1  &	17.8 / \textcolor{red}{\contour{red}{-}}1.6 &	48.2 / \textcolor{red}{\contour{red}{-}} 6.5 &	59.8 / \textcolor{red}{\contour{red}{-}}8.9 &	75.7 / \textcolor{red}{\contour{red}{-}}12.2  &	91.7 / \textcolor{red}{\contour{red}{-}}7.0
  &    & 	15.2 / \textcolor{red}{\contour{red}{-}}0.8 &	48.7 / \textcolor{red}{\contour{red}{-}}5.4 &	57.3 / \textcolor{red}{\contour{red}{-}}7.2 &	72.0 / \textcolor{red}{\contour{red}{-}}9.5 &	93.8 / \textcolor{red}{\contour{red}{-}}7.1                    \\ \bottomrule

\end{tabular}
}
\vspace{-8pt}
\caption{Results showing effectiveness of question filtering. For each dataset and model {\M}, we train $6$ question filters: five \FMTval{i}'s for $i \in \{0.3,0.5,0.6,0.7,0.9\}$ and one {\FM}. For a particular filter {\F} operating with {\MTM}, $\Delta$ (Pr/Re/F1) refers to the difference in (Pr/Re/F1) of {\F}${\langle{\tau_2}^*\rangle}{\rightarrow}${\MTM} and {\MTM}. $\%$ Filter refers to the $\%$ of questions preemptively discarded by the question filter. {\MTM} results for AQAD are relative to {\M}$\langle 0 \rangle$.}
\label{tab:main_table}
\end{table*}

==> EMNLP'21 Question Filtering/Tables/main_table_small.tex <==
\newfloatcommand{capbtabbox}{table}[][1.35\linewidth]

\begin{figure*}
\begin{floatrow}
\capbtabbox{%
    \setlength\extrarowheight{-6pt}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cccccccccccccc}
    \toprule
    & &   & \multicolumn{5}{c}{\textbf{{\M} : 12-Layer Transformer}}                                                                                                             &   & \multicolumn{5}{c}{\textbf{{\M} : 24-Layer Transformer}}                                                                                                                              \\ 
    & &     & \multicolumn{5}{c}{\textbf{{\F} : RoBERTa-Base }}                                                                                                             &   & \multicolumn{5}{c}{\textbf{{\F} : RoBERTa-Large }}                                                                                                                              \\ \cmidrule{4-8}
    \cmidrule{10-14} 
    \multicolumn{3}{c}{\centering \textbf{Threshold {\TM} for {\M} $\rightarrow$}}    & 0.3 & 0.5 & 0.6 & 0.7 & 0.9  &     & 0.3 & 0.5 & 0.6 & 0.7 & 0.9 \\ \toprule
    \multirow{9}{*}{\begin{turn}{90}\textbf{WikiQA}\end{turn}} & \multirow{2}{*}{{\MTM}} & Pr       	& 84.4  &	87.1  & 88.4  & 88.4  &	97.1  & & 92.1 	& 92.2 	& 92.0	& 92.1  &	95.9          \\ \cmidrule{3-3}
    & & Re       	&  80.2 &  75.3 & 68.7 &  63.0 &  28.0 & &   86.0	&  83.1	&  80.2	&  77.0 &	 57.2          \\ \cmidrule{2-3}
       & \multirow{2}{*}{\small{\FMTM${\langle{\tau_2^*}\rangle}{\rightarrow}${\M}$\langle${\TM}$\rangle$}}         & $\%$ Filter  & 4.1  & 2.9   & 3.7  & 7.0   & 42.8  &  &  0.8  & 3.3  & 6.6  & 7.8  & 18.9  \\ \cmidrule{3-3}
          &   & $\Delta$ Re   & \textcolor{red}{\contour{red}{-}}2.4  &  \textcolor{red}{\contour{red}{-}} 0.8  &  \textcolor{red}{\contour{red}{-}}1.6  &  \textcolor{red}{\contour{red}{-}}2.5  &  \textcolor{red}{\contour{red}{-}} 3.7 &  &   \textcolor{red}{\contour{red}{-}}0.8  &  \textcolor{red}{\contour{red}{-}}2.0  &  \textcolor{red}{\contour{red}{-}} 4.1  &  \textcolor{red}{\contour{red}{-}} 5.0  &  \textcolor{red}{\contour{red}{-}}6.1      \\ \cmidrule{2-3}
        
        & \multirow{2}{*}{\small{\FM${\langle{\tau_2^*}\rangle}{\rightarrow}${\M}$\langle${\TM}$\rangle$}}         & $\%$ Filter  & 4.1    & 17.3     & 20.9    & 21.0     & 44.0   &   &  1.2   & 1.8   & 2.6   & 3.9   & 8.8   \\ \cmidrule{3-3}
        &   & $\Delta$ Re   & \textcolor{red}{\contour{red}{-}}2.8  & \textcolor{red}{\contour{red}{-}}10.3  &  \textcolor{red}{\contour{red}{-}} 9.0  & \textcolor{red}{\contour{red}{-}}8.3  &  \textcolor{red}{\contour{red}{-}}7.4 &   &   \textcolor{red}{\contour{red}{-}}0.8  &  \textcolor{red}{\contour{red}{-}}0.8  &  \textcolor{red}{\contour{red}{-}}0.4  &  \textcolor{red}{\contour{red}{-}}2.1  &  \textcolor{red}{\contour{red}{-}}2.9  \\ \midrule
    %%%%%%%%%%%New Dataset
    \multirow{9}{*}{\begin{turn}{90}\textbf{ASNQ}\end{turn}} & \multirow{2}{*}{\MTM} & Pr                 & 68.2               & 74.6                 &           77.2                & 79.6        & 90.5   &   & 75.7             & 79.6     &         81.9             & 84.5                & 92.9       \\ \cmidrule{3-3}
     &  & Re                &   48.7                &   41.1                &           36.1              &   28.9      &  10.0 &   &   61.1               &   54.4    &          49.3            &   42.7               &  20.7     \\ \cmidrule{2-3}
        & \multirow{2}{*}{\small{\FMTM${\langle{\tau_2^*}\rangle}{\rightarrow}${\M}$\langle${\TM}$\rangle$}}         & $\%$ Filter        & 7.8        & 17.8           &     29.8   & 54.2                 & 83.8    &  & 0.2                              & 10.5    &     15.6         & 29.8     & 66.2      \\ \cmidrule{3-3}
        &  &  $\Delta$ Re         &  \textcolor{red}{\contour{red}{-}}1.8                &  \textcolor{red}{\contour{red}{-}}2.9               &      \textcolor{red}{\contour{red}{-}}4.7  &  \textcolor{red}{\contour{red}{-}}8.2                &   \textcolor{red}{\contour{red}{-}}3.9  &  &   0                              &  \textcolor{red}{\contour{red}{-}} 3.2  &     \textcolor{red}{\contour{red}{-}}3.0           &  \textcolor{red}{\contour{red}{-}}7.4               & \textcolor{red}{\contour{red}{-}}7.0                \\ \cmidrule{2-3}
        
        & \multirow{2}{*}{\small{\FM${\langle{\tau_2^*}\rangle}{\rightarrow}${\M}$\langle${\TM}$\rangle$}}         & $\%$ Filter         &  6.0   & 14.9    & 33.5    & 47.1    & 86.0  &  &  1.0   & 12.1   & 16.1  & 21.6    & 61.6    \\  \cmidrule{3-3}
    &   &  $\Delta$ Re         &   \textcolor{red}{\contour{red}{-}}1.2  &  \textcolor{red}{\contour{red}{-}}2.7  &  \textcolor{red}{\contour{red}{-}}5.3  &  \textcolor{red}{\contour{red}{-}}6.4  &  \textcolor{red}{\contour{red}{-}}5.1 &  &   \textcolor{red}{\contour{red}{-}}0.1  &  \textcolor{red}{\contour{red}{-}}3.3  &   \textcolor{red}{\contour{red}{-}}3.5  &  \textcolor{red}{\contour{red}{-}}3.9  &  \textcolor{red}{\contour{red}{-}}6.3   \\  \midrule
    % %%%%%%%%%%%New Dataset
    \multirow{9}{*}{\begin{turn}{90}\textbf{SQuAD 1.1}\end{turn}} & \multirow{2}{*}{{\MTM}} & Pr         &     	82.0    & 	88.7  & 	91.0   & 93.4   & 	96.7   &  & 	86.0 & 	90.1  & 	92.3  & 	94.4  & 	97.6         \\ \cmidrule{3-3}
     &  & Re         &     	  75.0  & 	 63.3 & 	  54.6 &  45.9 & 	 28.7 &  & 	 82.9 & 	 75.3 & 	 67.5 & 	 59.7 & 	 42.4         \\ \cmidrule{2-3}
        & \multirow{2}{*}{\small{\FMTM${\langle{\tau_2^*}\rangle}{\rightarrow}${\M}$\langle${\TM}$\rangle$}}         & $\%$ Filter         & 0   & 9.4    & 12.9   & 27.4  & 61.0    &   &  0  & 2.0    & 6.4  & 14.0  & 	47.5       \\ \cmidrule{3-3}
        &     &  $\Delta$ Re         & 0  & \textcolor{red}{\contour{red}{-}} 2.3  &  \textcolor{red}{\contour{red}{-}}2.4  &  \textcolor{red}{\contour{red}{-}}4.8  &   \textcolor{red}{\contour{red}{-}}7.7  &   &   0  &  \textcolor{red}{\contour{red}{-}}0.5  &  \textcolor{red}{\contour{red}{-}}1.8  &  \textcolor{red}{\contour{red}{-}}3.8 & 	 \textcolor{red}{\contour{red}{-}}3.7               \\ \cmidrule{2-3}    
        & \multirow{2}{*}{\small{\FM${\langle{\tau_2^*}\rangle}{\rightarrow}${\M}$\langle${\TM}$\rangle$}}         & $\%$ Filter            & 1.1   & 9.0    & 14.2    & 36.5    & 63.0   &      & 0   & 2.4  & 5.1  & 18.2   & 41.8   \\ \cmidrule{3-3} 
        &       &  $\Delta$ Re           &  \textcolor{red}{\contour{red}{-}}0.4  &  \textcolor{red}{\contour{red}{-}}2.3  &   \textcolor{red}{\contour{red}{-}}3.2  &  \textcolor{red}{\contour{red}{-}}8.2  &  \textcolor{red}{\contour{red}{-}}8.8 &      &  0 &  \textcolor{red}{\contour{red}{-}}0.5  &  \textcolor{red}{\contour{red}{-}}1.2 &  \textcolor{red}{\contour{red}{-}}5.5  &   \textcolor{red}{\contour{red}{-}}8.1  \\ \midrule 
    % %%%%%%%%%%%New Dataset
    \multirow{9}{*}{\begin{turn}{90}\textbf{AQAD} \end{turn}} & \multirow{2}{*}{\MTM} & Pr         &  	{$\uparrow$}9.2  & 	{$\uparrow$}17.9 & 	{$\uparrow$}23.4  & 	{$\uparrow$}28.1  & 	{$\uparrow$}43.0  &  &  	{$\uparrow$}9.2  & 	{$\uparrow$}17.9  & 	{$\uparrow$}23.4  & 	{$\uparrow$}28.1 & 	{$\uparrow$}43.0     \\ \cmidrule{3-3}
    &  &  Re         &  	 {$\downarrow$}4.5 & 	 {$\downarrow$}12.1 & 	 {$\downarrow$}15.7 & 	 {$\downarrow$}20.1 & 	 {$\downarrow$}31.9 &  &  	 {$\downarrow$}4.5 & 	 {$\downarrow$}12.1 & 	 {$\downarrow$}15.7 & 	 {$\downarrow$}20.1 & 	 {$\downarrow$}31.9     \\ \cmidrule{2-3}
        & \multirow{2}{*}{\small{\FMTM${\langle{\tau_2^*}\rangle}{\rightarrow}${\M}$\langle${\TM}$\rangle$}}         & $\%$ Filter            & 20.8    & 43.2    & 53.9    & 65.2    & 89.4   & &  21.9    & 45.8    & 56.9    & 66.2   & 89.9   \\ \cmidrule{3-3}
        &  & $\Delta$ Re           &  \textcolor{red}{\contour{red}{-}}3.4  &   \textcolor{red}{\contour{red}{-}}5.0  &   \textcolor{red}{\contour{red}{-}}5.6  &   \textcolor{red}{\contour{red}{-}}6.0  &   \textcolor{red}{\contour{red}{-}}3.4 & &    \textcolor{red}{\contour{red}{-}}3.2  &   \textcolor{red}{\contour{red}{-}}4.9  &  \textcolor{red}{\contour{red}{-}}5.5  &   \textcolor{red}{\contour{red}{-}}4.6  &  \textcolor{red}{\contour{red}{-}}3.0  \\ \cmidrule{2-3}    
        &\multirow{2}{*}{\small{\FM${\langle{\tau_2^*}\rangle}{\rightarrow}${\M}$\langle${\TM}$\rangle$}}  & $\%$ Filter   & 17.8   & 48.2    & 59.8    & 75.7    & 91.7   & & 15.2    & 48.7    & 57.3    & 72.0    & 93.8    \\ \cmidrule{3-3} 
        &  &  $\Delta$ Re          &  \textcolor{red}{\contour{red}{-}}2.8  &   \textcolor{red}{\contour{red}{-}}6.6  &   \textcolor{red}{\contour{red}{-}}7.5  &  \textcolor{red}{\contour{red}{-}}8.7  &   \textcolor{red}{\contour{red}{-}}3.8 & &   \textcolor{red}{\contour{red}{-}}1.7  &  \textcolor{red}{\contour{red}{-}}5.7  &  \textcolor{red}{\contour{red}{-}}6.2  &  \textcolor{red}{\contour{red}{-}}7.0  &   \textcolor{red}{\contour{red}{-}}3.9  \\ \bottomrule
    \end{tabular}
    }
}{%
    \caption{Filtering gains and drop in recall for question filters operating at optimal filtering threshold {\TFBest}. For a particular filter {\F} operating with answer model {\MTM}, $\Delta$ Re refers to the difference in Recall of {\F}${\langle{\tau_2}^*\rangle}{\rightarrow}${\MTM} and {\MTM}. $\%$ Filter refers to the $\%$ of questions preemptively discarded by {\F}. {\MTM} results for AQAD are relative to {\M}$\langle 0 \rangle$.}
    \label{tab:main_table_small} 
}
\centering
    \ffigbox[0.6\linewidth]
    {
    \begin{subfigure}[t]{0.95\linewidth}
        \includegraphics[width=0.87\linewidth]{Plots/Experiments/Filter_Threshold_Vary/asnq_0.5.png}
        \vspace{-0.15cm}
        \caption{{\small ASNQ}}
    \end{subfigure}
    \begin{subfigure}[t]{0.95\linewidth}
        \includegraphics[width=0.87\linewidth]{Plots/Experiments/Filter_Threshold_Vary/iqad_0.5.png}
        \vspace{-0.15cm}
        \caption{{\small AQAD}}
    \end{subfigure}
    }
    {
    \vspace{-0.25cm}
  \caption{$\Delta$ Pr/$\Delta$ Re plots and fraction of questions filtered on varying {\TF} for RoBERTa-Base {\FM}${\langle\tau_2\rangle}{\rightarrow}${\M}$\langle 0.5 \rangle$ on ASNQ and AQAD datasets.}
    \label{fig:threshold_vary_plots}
}
\end{floatrow}
\end{figure*}

==> EMNLP'21 Question Filtering/Tables/pr_re_graphs.tex <==
\begin{figure}[t]
\centering
    \begin{subfigure}[t]{\linewidth}
        \begin{subfigure}[t]{0.4825\textwidth}
            \includegraphics[width=1\textwidth]{Plots/Experiments/Pr_Re_Curves/squad.png}
            \caption{SQuAD 1.1}
        \end{subfigure}
        \begin{subfigure}[t]{0.5025\textwidth}
            \includegraphics[width=1\textwidth]{Plots/Experiments/Pr_Re_Curves/iqad.png}
            \caption{AQAD}
        \end{subfigure}
    \end{subfigure}
    \vspace{-3pt}
    \caption{Pr/Re curves for filters (\textcolor{blue}{\FM}, \textcolor{orange}{\FW}, \textcolor{magenta}{\FC}) and answer model \textcolor{red}{\M} (For AQAD we show $\Delta$Pr/$\Delta$Re w.r.t {\Mval{0}}). Since test splits only contain questions with at least one correct answer, Pr${=}$Re at {\TM}${=}0$.}
    \label{fig:pr_re_graphs}
    \vspace{-3pt}
\end{figure}
